Defending with Errors: Approximate Computing for Robustness of Deep Neural Networks

Machine-learning architectures, such as Convolutional Neural Networks (CNNs) are vulnerable to adversarial attacks: inputs crafted carefully to force the system output to a wrong label. Since machine-learning is being deployed in safety-critical and security-sensitive domains, such attacks may have catastrophic security and safety consequences. In this paper, we propose for the first time to use hardware-supported approximate computing to improve the robustness of machine-learning classifiers. We show that successful adversarial attacks against the exact classifier have poor transferability to the approximate implementation. Surprisingly, the robustness advantages also apply to white-box attacks where the attacker has unrestricted access to the approximate classifier implementation: in this case, we show that substantially higher levels of adversarial noise are needed to produce adversarial examples. Furthermore, our approximate computing model maintains the same level in terms of classification accuracy, does not require retraining, and reduces resource utilization and energy consumption of the CNN. We conducted extensive experiments on a set of strong adversarial attacks; We empirically show that the proposed implementation increases the robustness of a LeNet-5, Alexnet and VGG-11 CNNs considerably with up to 50% by-product saving in energy consumption due to the simpler nature of the approximate logic.

==> appx_bfloat.tex <==



==> theory.tex <==

%\begin{appendices}
% \section{Appendix: Theoretical Analysis} \label{sec:theory} %HEREx\nael{Need to come up with a better title for this section}
% %----------------------------------
% We now explore the impact of approximation on the classifier robustness leveraging some formulations from Differential Privacy (DP)~\cite{diff_priv}. %Before proceeding further, note that our purpose in this subsection is not to provide a definitive argument about using approximate computing to defend against adversarial attacks, but rather we view it as an initial step towards drawing an explanation that connects the circuit-level approximation to the model robustness for future work to build upon. 
% %Specifically, while the explainability of deep neural networks behavior is a challenging task, especially under adversarial settings, we attempt to provide an overview on the mechanisms that we think are behind the defensive approximation impact on security. 
% %\ihsen{Attempt starts here}\\
% Our formulation is based on recent similar formulations for certified robustness analysis~\cite{smooth,snP2019_certif}. These prior works studied the impact of randomization on robustness by adding random Gaussian noise to all layers of a CNN.%HEREx\nael{Random is imprecise -- is Gaussian accurate?  If not, what distributions of noise did they consider?} 
% While the noise injected by DA follows a different distribution and is input dependent rather than stochastic, we believe that the theoretical analysis provides insights into the possible mechanisms that improve the robustness of DA.
% %is a theoretical analogy with our work that we develop in the following.   

% In this analysis, we formally model the problem as follows:
% Let $x$ be an input sample and $h$ a conventional classifier. We denote $\hat{h}(x) = h(x) + \triangle(x)$ the defender implementation where $\triangle(x)$ is the data dependent randomness added by the approximate circuit. In this analysis, we use the concept of Differential Privacy (DP) \cite{diff_priv}, \cite{DP}, which is concerned whether the output of a computation over a given database can reveal information about individual records in the database. %In the context of insuring data privacy, these papers suggest injecting a level of randomness 
% To prevent such data leakage, randomness is introduced in the computation, and DP is accordingly defined as follows: 

% \begin{definition} 
%     A randomized algorithm $A$ that takes as input a database $d$ and outputs a value in a space $O$ is said to satisfy ($\varepsilon$, $\delta$)-DP w.r.t. a metric $\rho$ if, for any databases $d$ and $d^{\prime}$ with $\rho(d,d^{\prime}) \leqslant1$, and for any subset of possible outputs $S \subseteq O$, we have:
%     \begin{equation}
%         P(A(d) \in S) \leq e^{\varepsilon} P\left(A\left(d^{\prime}\right) \in S\right)+\delta
%     \end{equation}
% \end{definition}

% Out of this definition, Expected Output Stability Bound, a key property of DP is deduced; the expected value of an ($\varepsilon$, $\delta$)-DP algorithm with bounded output is not sensitive to small changes in the input.
% %\ihsen{next lemma needs more introduction, to match randomization to approximation. A small figure would be perfect. UPDATE: actually we do not need to bring this Lemma here. Go directly to corollary! UPDATE: Nope, the rest of the logic doesn't make sense. Keep it -for now-}


% % \begin{lemma}
% % \label{lemma1}
% % Suppose a randomized function $A$, with bounded output $A(x) \in [0, b], b \in \mathbb{R}^{+}$, satisfies $(\varepsilon, \delta)$-DP. Then the expected output meets the following property: 
% % \begin{center}
% %     $\forall \alpha \in B_{p}(1) . \mathbb{E}(A(x)) \leq e^{\epsilon} \mathbb{E}(A(x+\alpha))+b \delta$
% % \end{center}
% % \end{lemma}

% The intuition behind using the analogy with DP in the context of robustness to adversarial examples is to create an approximate classifier such that, given an input example, the predictions are DP with regards to the features of the input (e.g., the pixels of an image). In this setting, we can derive stability bounds for the expected output of the randomized classifier, i.e., the approximate classifier. The bounds can be interpreted as a certification for robustness to adversarial examples. In our method, the added approximate noise $\triangle(x)$ for a given input $x$ has a similar effect to randomization.


% Formally, to frame the DP into our setting, regard the feature values (e.g., pixels) of an input $x$ as the records in a database.  Let $B_{p}(r):=\left\{\alpha \in \mathbb{R}^{n}:\|\alpha\|_{p} \leq r\right\}$ be the $p$-norm ball of radius $r$. For a given classification model, $h$, and a fixed input, $x \in \mathbb{R}
% ^n$, an attacker is able to craft a successful adversarial example of size $L$ for a given $p$-norm if they find $\alpha \in  B_{p}(L)$ such that $h(x + \alpha) \neq h(x)$. Now, consider an approximate classifier $\hat{h}$ that, on input $x$, outputs scores $\left(y_{1}(x), \ldots, y_{K}(x)\right) \text { (with } y_{k}(x) \in[0,1]$ and $\sum_{k=1}^{K} y_{k}(x)=1)$. 


% Combining Lemma $1$ and Corollary $1$ in \cite{snP2019_certif} directly implies bounds on the expected output on an approximate classifier:
% \begin{theorem}
% Suppose an approximate function $\hat{h}$ satisfies $(\varepsilon, \delta)$-DP w.r.t. a $p$-norm metric, and where $\hat{h}(x)=\left(y_{1}(x), \ldots, y_{K}(x)\right), y_{k}(x) \in[0,1]$:
% \begin{equation}
% \label{eq:dp}
%     \forall k, \forall \alpha \in B_{p}(1) . \hat{h}_{k}(x) \leq e^{\varepsilon} \hat{h}_{k}(x+\alpha) +\delta.%~ \footnote{This corollary and the detailed proofs can be found in \cite{snP2019_certif}} 
% \end{equation}
% \end{theorem}

% Now, consider $\alpha \in B_p(1)$, and let $x^* = x + \alpha$. From Equation \ref{eq:dp}, we have: \textbf{(i)} $\hat{h}_{k}(x) \leqslant e^\varepsilon \hat{h}_{k}(x^*) + \delta$, and
% \textbf{(ii)} $\hat{h}_{i\neq k}(x^*) \leqslant e^\varepsilon \hat{h}_{i\neq k}(x) + \delta$.

% Practically, \textbf{(i)} gives a lower-bound on $\hat{h}_{k}(x^*)$ and \textbf{(ii)} gives an upper-bound on  $\hat{h}_{i\neq k}(x^*)$.

% These elements confirm a theoretically verifiable bounded impact of an adversarial perturbation in the input on the approximate classifier's output. 


% To further investigate the robustness guarantee, suppose that when the base classifier $h$ classifies an input $x$ the most probable class $k$ is returned with probability $p_k$, and the “runner-up” class is returned with probability $p_{i\neq k}< p_k$. Based on \cite{smooth}, our approximate classifier is robust around $x$ within the $\ell_{2} \text { radius } R=\frac{\sigma}{2}\left(\Phi^{-1}\left(p_{k}\right)-\Phi^{-1}\left(p_{i}\right)\right)$, where $\Phi^{-1}$ is the inverse of the standard Gaussian CDF. This result also holds if we replace $p_k$ with a lower bound $\underline{{p}_{k}}$  and we replace $p_i$ with an upper bound $\overline{p_{B}}$. Hence, based on Theorem 1 in \cite{smooth}:

% \begin{theorem}
% \label{theorem:smooth}
% Let  $h: \mathbb{R}^{d} \rightarrow \mathcal{Y}$ be any baseline classifier, and let $\varepsilon \sim \mathcal{N}\left(0, \sigma^{2} I\right)$. Let $\hat{h}$ be the approximate implementation of $h$. Suppose $c_{k} \in \mathcal{Y} \text { and } \underline{p_{k}}, \overline{p_{i}} \in[0,1]$ satisfy:

% \begin{equation}
%     \mathbb{P}\left(h(x+\varepsilon)=c_{k}\right) \geq \underline{p}_{k} \geq \overline{p_{i}} \geq \max _{c \neq c_{k}} \mathbb{P}(h(x+\varepsilon)=c)
% \end{equation}

% Then $\hat{h}(x+ \delta) = c_k$ for all $\|\delta\|_{2}<R$, where 
% \begin{equation}
% \label{eq:theorem_smooth}
%     R=\frac{\sigma}{2}\left(\Phi^{-1}\left(\underline{p_{k}}\right)-\Phi^{-1}(\overline{p_{i}})\right)
% \end{equation}

% \end{theorem}

% Notice that Theorem \ref{theorem:smooth} insures a certified radius $R$ that is large when: (1) the noise level $\sigma$ is high, (2) the probability of the top class $c_k$ is high, and (3) the probability of each other class $c_{i \neq k}$ is low.

% Conditions (2) and (3) of high radius basically mean a higher confidence in the sense of Equation \ref{eq:confidence}. This is coherent with the results obtained in terms of robustness, given Figure \ref{conf_dis}.

% The randomization technique proposed in \cite{snP2019_certif} and \cite{smooth} uses a totally random noise that is uncorrelated to the input. This led them to use heavy Monte Carlo simulations to estimate the randomized classifier's output, which induces a considerable time overhead limiting the applicability of these techniques, especially in time critical applications. In our approach, the noise is injected at circuit-level through the approximate design and is not artificially generated from an outside source. Moreover, the correlation to the input that highlights useful features in the convolution output gives higher confidence and thereby ensures a higher robustness radius in the sense of Theorem \ref{theorem:smooth}.

\section{Appendix: Design Space Exploration} \label{sec:DSE}
\textbf{Accuracy.} HEAP \cite{Heap} is the result of a design space exploration among combinations of different approximate full adders leading to minimal accuracy loss. The selection process of optimal circuit design was performed after an exhaustive accuracy evaluation of all possible configurations.% The exploration was performed as described in \textbf{Algorithm 1}
The metrics used to evaluate the accuracy of different combinations are the mean relative error distance (MRED) \cite{metrics} $ {\textstyle MRED= \frac{1}{n} \sum_{i=1}^{n} \frac{ \mid{\hat Y -Y}\mid}{Y} }$, and the normalized mean error distance (NMED): ${\textstyle NMED= \frac{1}{n} \sum_{i=1}^{n} \frac{ \mid{\hat Y -Y}\mid}{P_{max}} }$. Where $Y$ is the exact result, $ \hat Y $ is the approximate result, and $P_{max}$ is the maximum product.

%\begin{algorithm}
%\caption{DSE Algorithm}
%\begin{algorithmic}[1]
%\State \textbf{Input:} POPSIZE //size of the population;\\
%C //Error constraint;
%\State \textbf{Output:} final combination
%%\textit{//Initialize population:}
%\State i = 0;
%\While {i < POPSIZE}
%\State Generate random combination;
%\State Calculate the NMED;
%\If {NMED < C}
%\State Add the new combination to the population;
%\State i++;
%\EndIf
%\EndWhile
%%\State \textit{//Minimize fitness function:}
%\Repeat
%\State Calculate the fitness of each combination;
%\State Sort population according to fitness;
%%\State \textit{//Generate new population:}
%\State Select the \textit{best} individuals to reproduce;
%\State Generate new offspring using crossover and mutation
%\State Calculate the NMED of the new offspring;
%\If {NMED < C}
%\State Add the offspring to the new population;
%\EndIf
%\Until no improvement
%\end{algorithmic}
%\end{algorithm}
\begin{table}[!htp]
\centering
  \caption{Accuracy results of the LeNet-5 CNN and different multipliers.}
  \label{tab3_}
  \begin{tabular}{cccc}
    \toprule
    \textbf{Multiplier }& \textbf{CNN Accuracy}	& \textbf{MRED} & \textbf{NMED}	 \\
    \midrule
        Exact multiplier        & 97.93\%  & 0    & 0\\
        HEAP \cite{Heap}        & 97.86\%  & 0.12 & 0.03\\
        Ax-FPM	    & 97.67\%  & 0.33 & 0.08\\ 
  \bottomrule
\end{tabular}
\end{table}

Table \ref{tab3_} includes the accuracy results of the exact multiplier and the two approximate multipliers.
Ax-FPM is substantially less accurate than HEAP.  However, when we evaluate CNN accuracy (using the recognition rate), we notice a negligible accuracy loss for both approximate multipliers, confirming the inherent error-resiliency of CNNs.

\begin{figure}[!htp]
\centering
\includegraphics[width=0.9\columnwidth,height=3.5cm]{figures/error_dis (8).pdf}
\caption{Noise introduced by the approximate multiplier while the operands $\in [0,1]$ (a). for Ax-FPM, (b). for HEAP \cite{Heap}. 
}
\label{appx_mult_heap}
\end{figure}
Measuring the error introduced by the Ax-FPM and the HEAP for small inputs ranging between $0$ and $1$, see Figure \ref{appx_mult_heap}, we notice that, in addition to the smaller magnitude of error when using the HEAP, a different pattern was found: less data dependency and for only $34\%$ of the cases, the HEAP results were higher than the exact multiplier results. 

In order to further investigate the impact of different approximate multipliers on the convolution layer output, we produce different heat maps. As shown in Figure \ref{heatmaps}, we can see that the Ax-FPM is further highlighting the important features by increasing their scores whereas the HEAP is lowering their scores.

\begin{figure}[!htp]
\centering
\includegraphics[width=0.9\columnwidth]{figures/Heatmaps.pdf}
\caption{ Heat maps of final convolution layer output when using Exact multiplier, Ax-FPM, and HEAP \cite{Heap}. }
\label{heatmaps}
\end{figure}

\noindent\textbf{Energy consumption and Delay.}
We also compare the gain in terms of energy and delay achieved by the two approximate mantissa multipliers. Multipliers are implemented using $45~ n m$ technology via the Predictive Technology Model (PTM) using the Keysight Advanced Design System (ADS) simulation platform~\cite{ptm}.   

\begin{table}[!htp]
\centering
  \caption{Energy and delay of different $24\times24$ approximate multipliers normalized to a conventional $24\times24$ multiplier.}
  \label{tab}
  \begin{tabular}{ccc}
    \toprule
    \textbf{Multiplier }& \textbf{Average energy}	& \textbf{Average delay}  	 \\
    \midrule
        Exact multiplier        & 1 & 1    \\
        HEAP                    & 0.49  & 0.46\\
        Ax-FPM	                 & 0.395 & 0.235\\ 
  \bottomrule
\end{tabular}
\end{table}

As shown in Table \ref{tab}, the mantissa multiplier in Ax-FPM achieves a considerable gain in performance and energy saving compared to the HEAP. A significant reduction in the delay was also achieved.  

\noindent\textbf{Robustness.}
We tried to assess different models transferability, the adversarial examples were generated to fool the exact model. In table \ref{grey-boxresult_with_heap}, we present the percentage of adversarial examples that successfully deceived the approximate models. While the use of the HEAP increased the robustness of the model, the Ax-FPM achieved better results.

\begin{table}[!htp]
\small
\centering
  \caption{Attacks transferability success rates for MNIST.}
  \label{grey-boxresult_with_heap}
  \begin{tabular}{cccc}
    \toprule
    \textbf{Attack} & \textbf{Exact-based}  & \textbf{HEAP-based} & \textbf{Ax-FPM-based}\\
    \midrule
        FGSM          &   100\%  & 16\% & 12\%    \\
        PGD           &   100\%  & 30\% & 28\%    \\
        JSMA          &   100\%  & 42\% & 9\%   \\
        C\&W          &   100\%  & 6\% & 1\%    \\
        DF	          &   100\%  & 18\%  & 17\%   \\ 
        LSA	          &   100\%  & 41\% & 18\%   \\ 
        BA	          &   100\%  & 22\% & 17\%   \\ 
        HSJ	          &   100\%  & 4\% & 2\%    \\         
  \bottomrule
\end{tabular}
\end{table}

All these results confirm that Ax-FPM is a better choice in terms of robustness and resource and power efficiency.

\section{Appendix: Defensive Quantization: Models Architecture}
\label{mod_archi}
We present models architectures in Table \ref{architecture}: For the fully quantized model, ConvolutionQuant, DenseQuant and reluQuant designate respectively a convolution layer with quantized weights, a dense layer with quantized weights and the relu activation function with its output quantized. For the weight quantized model architecture, the ConvolutionQuant and DenseQuant designate respectively a convolution layer with quantized weights and a dense layer with quantized weights.

\begin{table}[!htp]
\small
\centering
  \caption{Fully quantized and Weight quantized models architecture.}
  \label{architecture}
  \begin{tabular}{cc}
    \toprule
    \textbf{Fully Quantized} & \textbf{Weight Quantized}  \\
    \midrule
        ConvolutionQuant     &  ConvolutionQuant    \\
        BatchNorm            &  BatchNorm   \\
        reluQuant            &  relu    \\
        ConvolutionreluQuant &  ConvolutionreluQuant    \\
        MaxPooling           &  MaxPooling    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant            &  relu  \\
        ConvolutionQuant     &  ConvolutionQuant    \\
        BatchNorm            &  BatchNorm     \\
        reluQuant            &  relu \\
        ConvolutionQuant     &  ConvolutionQuant    \\
        MaxPooling           &  MaxPooling    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant            &  relu \\
        ConvolutionQuant     &  ConvolutionQuant    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant            &  relu\\
        ConvolutionQuant     &  ConvolutionQuant    \\
        MaxPooling           &  MaxPooling    \\ 
        BatchNorm            &  BatchNorm    \\
        reluQuant            &  relu    \\
        DenseQuant           &  DenseQuant    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant       	 &  relu   \\ 
        DenseQuant           &  DenseQuant    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant	         &  relu    \\ 
        Dense                &  Dense    \\
        softmax	             &  softmax    \\ 
               
  \bottomrule
\end{tabular}
\end{table}

%\end{appendices}
